Bridging Memory Gaps: Scaling Federated Learning for Heterogeneous Clients

Federated Learning (FL) enables multiple clients to collaboratively train a shared model while preserving data privacy. However, the high memory demand during model training severely limits the deployment of FL on resource-constrained clients. To this end, we propose \our, a scalable and inclusive FL framework designed to overcome memory limitations through sequential block-wise training. The core idea of \our is to partition the global model into blocks and train them sequentially, thereby reducing training memory requirements. To mitigate information loss during block-wise training, \our introduces a Curriculum Mentor that crafts curriculum-aware training objectives for each block to steer their learning process. Moreover, \our incorporates a Training Harmonizer that designs a parameter co-adaptation training scheme to coordinate block updates, effectively breaking inter-block information isolation. Extensive experiments on both simulation and hardware testbeds demonstrate that \our significantly improves model performance by up to 84.2\%, reduces peak memory usage by up to 50.4\%, and accelerates training by up to 1.9$\times$.

==> Figure/Fig_robust.tex <==
\definecolor{red}{RGB}{172,21,28}
\definecolor{blue}{RGB}{39,89,167}
\definecolor{red1}{RGB}{203,104,104}
\definecolor{blue1}{RGB}{104,155,203}
\definecolor{color1}{RGB}{235,164,122}
\definecolor{color3}{RGB}{78,172,183}
\definecolor{color2}{HTML}{95a792}

\begin{figure}[t]
    \centering
    \vspace{1.0mm}
\begin{tikzpicture}
    \scriptsize{

  \begin{axis}[
    at={(-5.5em,-15.5em)},
    anchor=south west,
    ymajorgrids,
    grid style=dashed,
    legend style={at={(0.02,1)}, anchor=south west},
    legend cell align={left},
    ybar,
    enlarge x limits=0.5,
    xtick align=inside,
    height=.23\textwidth,
    width=.27\textwidth,
    bar width=1.3em,
    xlabel={\scriptsize{(a) CIFAR10}},
    xlabel style={scale=1.2, yshift=0.8em, xshift=0.1em},
    ylabel=\footnotesize{\scriptsize Accuracy (\%)},
    ylabel style={scale=1.2, yshift=0.3em},
    symbolic x coords={{1}, {2},},
    xtick=data,
    ymin=75,
    ymax=92,
    ytick={75,80,85,90,95},
    nodes near coords align={vertical},
    xticklabels={IID, Non-IID},
    ylabel style={yshift=-2em},
    yticklabel style={/pgf/number format/fixed,/pgf/number format/fixed zerofill,/pgf/number format/precision=0,rotate=0,scale=1.0},
    legend style={yshift=0.2em,xshift=4.2em,font={\tiny},cells={anchor=west},fill opacity=0.8, scale=1.0, legend columns=3}
    ]
    \addplot[fill=color1, draw=color1, area legend] coordinates {({1},67.0) ({2},76.8)};
    \addlegendentry{\scalebox{1.0}{{FedAvg}}}
    \addplot[fill=color2, draw=color2, area legend] coordinates {({1},0.0) ({2},78.2)};
    \addlegendentry{\scalebox{1.0}{\textsc{SBT}}}
    \addplot[fill=color3, draw=color3, area legend] coordinates {({1},80.1) ({2},88.4)};
    \addlegendentry{\scalebox{1.0}{\textsc{TheoFL}}}
    
    \addplot[fill=color3, draw=color3, area legend] coordinates {({1},9.9) ({2},88.4)};
    \addlegendentry{\scalebox{1.0}{\textsc{TheoFL}}}

    \addplot[fill=color3, draw=color3, area legend] coordinates {({1},81.4) ({2},88.4)};
    \addlegendentry{\scalebox{1.0}{\textsc{TheoFL}}}

    \addplot[fill=color3, draw=color3, area legend] coordinates {({1},82.0) ({2},88.4)};
    \addlegendentry{\scalebox{1.0}{\textsc{TheoFL}}}

    \addplot[fill=color3, draw=color3, area legend] coordinates {({1},82.5) ({2},88.4)};
    \addlegendentry{\scalebox{1.0}{\textsc{TheoFL}}}

    \addplot[fill=color3, draw=color3, area legend] coordinates {({1},84.2) ({2},88.4)};
    \addlegendentry{\scalebox{1.0}{\textsc{TheoFL}}}
  \end{axis}
	
  \begin{axis}[
    at={(11.5em,-15.5em)},
    anchor=south west,
    ymajorgrids,
    grid style=dashed,
    legend style={at={(0.02,1)}, anchor=south west},
    legend cell align={left},
    ybar,
    enlarge x limits=0.5,
    xtick align=inside,
    height=.23\textwidth,
    width=.27\textwidth,
    bar width=1.3em,
    xlabel={\scriptsize{(a) CIFAR100}},
    xlabel style={scale=1.2, yshift=0.8em, xshift=0.1em},
    ylabel=\footnotesize{\scriptsize Accuracy (\%)},
    ylabel style={scale=1.2, yshift=0.3em},
    symbolic x coords={{1}, {2},},
    xtick=data,
    ymin=30,
    ymax=63,
    ytick={30,40,50,60},
    nodes near coords align={vertical},
    xticklabels={IID, Non-IID},
    ylabel style={yshift=-2em},
    yticklabel style={/pgf/number format/fixed,/pgf/number format/fixed zerofill,/pgf/number format/precision=0,rotate=0,scale=1.0},
    legend style={yshift=0.2em,xshift=4.2em,font={\tiny},cells={anchor=west},fill opacity=0.8, scale=1.0, legend columns=3}
    ]
    \addplot[fill=color1, draw=color1, area legend] coordinates {({1},37.1) ({2},35.2)};
    % \addlegendentry{\scalebox{1.0}{\textsc{FedAvg}}}
    \addplot[fill=color2, draw=color2, area legend] coordinates {({1},54.4) ({2},48.2)};
    % \addlegendentry{\scalebox{1.0}{\textsc{Sequential}}}
    \addplot[fill=color3, draw=color3, area legend] coordinates {({1},59.6) ({2},58.1)};
    % \addlegendentry{\scalebox{1.0}{\textsc{TheoFL}.}}
  \end{axis}
}   
\end{tikzpicture}
\vspace{-5mm}
\caption{
Performance comparison on ResNet34.
}
\label{fig:robust}
\vspace{-4mm}
\end{figure}


==> Section/checklist.tex <==
% \newpage
\section{Reproducibility Checklist}

\textbf{Question1:} Includes a conceptual outline and/or pseudocode description of AI methods introduced? \\
Answer: Yes. \\
\textbf{Question2:} Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results? \\
Answer: Yes. \\
\textbf{Question3:} Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper? \\
Answer: Yes. \\
\textbf{Question4:} Does this paper make theoretical contributions? \\
Answer: Yes. \\
\textbf{Question5:} All assumptions and restrictions are stated clearly and formally? \\
Answer: Yes. \\
\textbf{Question6:} All novel claims are stated formally (e.g., in theorem statements)? \\
Answer: Yes. \\
\textbf{Question7:} Proofs of all novel claims are included? \\
Answer: Yes. \\
\textbf{Question8:} Proof sketches or intuitions are given for complex and/or novel results? \\
Answer: Yes. \\
\textbf{Question9:} Appropriate citations to theoretical tools used are given? \\
Answer: Yes. \\
\textbf{Question10:} All theoretical claims are demonstrated empirically to hold? \\
Answer: Yes. \\
\textbf{Question11:} All experimental code used to eliminate or disprove claims is included? \\
Answer: Yes. \\
\textbf{Question12:} Does this paper rely on one or more datasets? \\
Answer: Yes. \\
\textbf{Question13:} A motivation is given for why the experiments are conducted on the selected datasets? \\
Answer: Yes. \\
\textbf{Question14:} All novel datasets introduced in this paper are included in a data appendix? \\
Answer: Yes. \\
\textbf{Question15:} All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes? \\
Answer: NA. \\
\textbf{Question16:} All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations? \\
Answer: Yes. \\
\textbf{Question17:} All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available? \\
Answer: Yes. \\
\textbf{Question18:} All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing? \\
Answer: NA. \\
\textbf{Question19:} Does this paper include computational experiments? \\
Answer: Yes. \\
\textbf{Question20:} This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting? \\
Answer: Yes. \\
\textbf{Question21:} Any code required for pre-processing data is included in the appendix? \\
Answer: Yes. \\
\textbf{Question22:} All source code required for conducting and analyzing the experiments is included in a code appendix? \\
Answer: Yes. \\
\textbf{Question23:} All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes? \\
Answer: Yes. \\
\textbf{Question24:} All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from ? \\
Answer: Yes. \\
\textbf{Question25:} If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results? \\
Answer: Yes. \\
\textbf{Question26:} This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks? \\
Answer: Yes. \\
\textbf{Question27:} This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics? \\
Answer: Yes. \\
\textbf{Question28:} This paper states the number of algorithm runs used to compute each reported result? \\
Answer: Yes. \\
\textbf{Question29:} Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information? \\
Answer: Yes. \\
\textbf{Question30:} The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank)? \\
Answer: Yes. \\
\textbf{Question31:} This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments? \\
Answer: Yes. \\


==> Section/new_checklist.tex <==
\section*{Reproducibility Checklist}
\newcommand{\answerYes}{\textbf{yes}}
\newcommand{\answerNO}{\textbf{no}}
\newcommand{\answerNA}{\textbf{NA}}

Unless specified otherwise, please answer ``yes" to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled ``Reproducibility Checklist'' at the end of the technical appendix.

\subsection*{This paper:}

\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA)\\
    Answer: \answerYes{}
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no)\\
    Answer: \answerYes{}
    \item Provides well marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper (yes/no)\\
    Answer: \answerYes{}
\end{itemize}

\subsection*{Does this paper make theoretical contributions? (yes/no) If yes, please complete the list below.}
Answer: \answerYes{}


\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)\\
    Answer: \answerYes{}
    \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)\\
    Answer: \answerYes{}
    \item Proofs of all novel claims are included. (yes/partial/no)\\
    Answer: \answerYes{}
    \item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)\\
    Answer: \answerYes{}
    \item Appropriate citations to theoretical tools used are given. (yes/partial/no)\\
    Answer: \answerYes{}
    \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)\\
    Answer: \answerYes{}
    \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)\\
    Answer: \answerYes{}
\end{itemize}

\subsection*{Does this paper rely on one or more datasets? (yes/no)}
Answer: \answerYes{}

\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA)\\
    Answer: \answerYes{}
    \item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA)\\
    Answer: \answerNA{}
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA)\\
        Answer: \answerNA{}
    \item All datasets drawn from the existing literature (potentially including authors' own previously published work) are accompanied by appropriate citations. (yes/no/NA)\\
    Answer: \answerYes{}
    \item All datasets drawn from the existing literature (potentially including authors' own previously published work) are publicly available. (yes/partial/no/NA)\\
    Answer: \answerYes{}
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisfying. (yes/partial/no/NA)\\
    Answer: \answerNA{}
\end{itemize}

\subsection*{Does this paper include computational experiments? (yes/no)}
Answer: \answerYes{}

\begin{itemize}
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA)\\
    Answer: \answerYes{}
    \item Any code required for pre-processing data is included in the appendix. (yes/partial/no)\\
    Answer: \answerYes{}
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no)\\
    Answer: \answerYes{}
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no)\\
        Answer: \answerYes{}
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no)\\
    Answer: \answerYes{}
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA)\\
    Answer: \answerYes{}
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no)\\
        Answer: \answerYes{}
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no)\\
    Answer: \answerYes{}
    \item This paper states the number of algorithm runs used to compute each reported result. (yes/no)\\
    Answer: \answerYes{}
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no)\\
        Answer: \answerYes{}
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no)\\
    Answer: \answerYes{}
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper's experiments. (yes/partial/no/NA)\\
    Answer: \answerYes{}
\end{itemize}
